Inline Vector Compression for Computational Physics

A novel inline data compression method is presented for single-precision vectors in three dimensions. The primary application of the method is for accelerating computational physics calculations where the throughput is bound by memory bandwidth. The scheme employs spherical polar coordinates, angle quantisation, and a bespoke floating-point representation of the magnitude to achieve a fixed compression ratio of 1.5. The anisotropy of this method is considered, along with companding and fractional splitting techniques to improve the efficiency of the representation. We evaluate the scheme numerically within the context of high-order computational fluid dynamics. For both the isentropic convecting vortex and the Taylor--Green vortex test cases, the results are found to be comparable to those without compression. Performance is evaluated for a vector addition kernel on an NVIDIA Titan V GPU; it is demonstrated that a speedup of 1.5 can be achieved.

==> app_precision.tex <==
%!TEX root = ./vecc_main.tex
\section{Intermediate Precision Analysis}
\label{sec:app_precision}

Consider some vector $\mathbf{x} \in V^3$, where $V \subset \mathbb{R}$ is the set of floating-point numbers with an $n$ bit exponent and $m$ bit mantissa. Let us define a compression and subsequent decompression as a function such that $f: V^3 \rightarrow U^3_1$. Where $U_1^3$ is the result of one compression decompression cycle. It should be clear that by definition $U_n^3 \subset V^3$. An important property that we wish to understand is weather the compression-decompression transformation $f$ is idempotent, $f: U^3_n \rightarrow U^3_{n+1}$ and $U_n^3 = U^3_{n+1}$. To understand this let us define a point: $\mathbf{x}_i \in U^3_i$ for $i\geqslant1$. Therefore, we wish for $\mathbf{x}_n = \mathbf{x}_{n+1}$ and it will be sufficient examine $n_{\theta,n}$, $n_{\theta,n+1}$, $n_{\phi,n}$, and $n_{\phi,n+1}$. From Eq.~(\ref{eq:a_disc}) we can define:
	\begin{align*}
		n_{\theta,n} =&\: \sceil{\Bigg}{\frac{\sfloor{\Big}{\frac{n_{\theta,\mathrm{max}}\big[\tan^{-1}{\big(\frac{y_{n-1}}{x_{n-1}}\big)} + \pi\big]}{\pi}}}{2}} \\
		n_{\theta,n+1} =&\: \sceil{\Bigg}{\frac{\sfloor{\Big}{\frac{n_{\theta,\mathrm{max}}\big[\tan^{-1}{\big(\frac{y_{n}}{x_{n}}\big)} + \pi\big]}{\pi}}}{2}}.
	\end{align*}
	We want $n_{\theta,n} = n_{\theta,n+1}$, which in turn implies:
	\[
		\sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\big[\tan^{-1}{\big(\frac{y_{n-1}}{x_{n-1}}\big)} + \pi\big]}{\pi}} = \sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\big[\tan^{-1}{\big(\frac{y_{n}}{x_{n}}\big)} + \pi\big]}{\pi}}
	\] 
	If it is then assumed that the error in the addition is negligible then:
	\[
		\sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\tan^{-1}{\big(\frac{y_{n-1}}{x_{n-1}}\big)}}{\pi}} = \sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\tan^{-1}{\big(\frac{y_{n}}{x_{n}}\big)}}{\pi}}
	\] 
	An error term may be introduced into the left and right terms that gives the tolerance of the equality:
	\begin{equation}\label{eq:tol1}
		\sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\tan^{-1}{\big(\frac{y_{n-1}}{x_{n-1}}\big)}}{\pi} + \alpha_n} = \sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\tan^{-1}{\big(\frac{y_{n}}{x_{n}}\big)}}{\pi} + \alpha_{n+1}} 
	\end{equation}
	where $\alpha_i \in [-1,1]$. The exact bound of the tolerance will be dependent on the value of $\tan^{-1}$ and is what we will now find. First we will reformulate Eq.~(\ref{eq:tol1}) to:
	\[
		\sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\big[\tan^{-1}{\big(\frac{y_{n-1}}{x_{n-1}}\big) + \frac{n_{\theta,\mathrm{max}}\alpha_n}{\pi}\big]}}{\pi}} = \sfloor{\bigg}{\frac{n_{\theta,\mathrm{max}}\big[\tan^{-1}{\big(\frac{y_{n}}{x_{n}}\big) + \frac{n_{\theta,\mathrm{max}}\alpha_{n+1}}{\pi}\big]}}{\pi}}
	\]
	Therefore, if the error induced by $\tan^{-1}(y/x)$ is:
	\[
		\tan^{-1}(y/x) = \tan^{-1}(y/x)(1 \pm u2^{-m})
	\]
	where $u$ is the number of ULPs to which the arc-tangent is calculated and $m$ is the number of mantissa bits for the calculation precision. Typically, for inverse trigonometric functions, $u \in\{x\in\mathbb{N}| x<10\}$. Then, when:
	\begin{equation}
		|\alpha_n| > u2^{p-m}
	\end{equation}	 
	the compression method will be idempotent, where $n_{\theta,\mathrm{max}} = 2^p$. The interpretation of this is that the error in the arc-tangent is amplified and so angles that are within in $u2^{p-m}$ of the floor can be moved into the next bracket. For example, if $p=16$ and $m=24$ then $|\alpha| > u/256$. The implication is that $2u/256$ as a fraction of angles will not be idempotent, a characteristic which may impact the accuracy of the underlying numerical method. Similar analysis may be repeated for $n_\phi$ yielding a similar result. To mitigate this, and to ensure the arithmetic error is lower than the quantisation error, sufficient precision must be used in the intermediaries of inverse trigonometric functions. In the context of this scheme this means the use of double precision arithmetic.  
